Control-Tutored Reinforcement Learning: Towards the Integration of Data-Driven and Model-Based Control

We present an architecture where a feedback controller derived on an approximate model of the environment assists the learning process to enhance its data efficiency. This architecture, which we term as Control-Tutored Q-learning (CTQL), is presented in two alternative flavours. The former is based on defining the reward function so that a Boolean condition can be used to determine when the control tutor policy is adopted, while the latter, termed as probabilistic CTQL (pCTQL), is instead based on executing calls to the tutor with a certain probability during learning. Both approaches are validated, and thoroughly benchmarked against Q-Learning, by considering the stabilization of an inverted pendulum as defined in OpenAI Gym as a representative problem.

==> figures/Block_Schema.tex <==
\begin{figure}[htbp]
\vspace{0.3cm}
\hspace*{1em}
\centering
\begin{tikzpicture}[auto, node distance=1.8cm]
    \node [input, name=input] {};
    \node [block, right of=input] (system) {System};
    % \node [block, below of=system, right of=system, xshift=1cm] (RF) {Reward Function};
    \node [block, below of=system, xshift=-3cm , yshift=-2cm, text width=2.3cm] (RL) {Reinforcement Learning};
    \node [block, below of=RL] (CT) {Control Tutor};
    % \node [block, below of=system, left of=system, xshift=-2cm] (policyQ) {\large $\pi^R$};
    % \node [block, below of=system, left of=system, xshift=-4.4cm] (policyT) {\large $\pi^C$};
    % \node [block, below of=policyT, yshift=-0.4cm] (CL) {Control Law};

    %\draw [->] (system.est) -| node [pos=0.25] [name=S] {$x_{k+1},x_{k}$} (RL);
    \draw [-] (system) --  ++(1.4cm,0) coordinate(S1) {};
    \draw [->] (S1) -- node [pos=0.3] [name=A1] [above] {$x_{k}$} ++(0.5cm,0) coordinate(S2) {};
    \draw [-] (S1) |-  ++(0,-4.05cm) coordinate(S2) {};
    \draw [->] (S2) |-  ++(-3.11cm,0) coordinate(S3);
    \draw [->] (S2) |-  (CT);
    % \draw [->] (RF) |-  node [pos=0.1] {$r_{k+1}$} (LU);
    % \draw [->] (S1) |- (Q);
    % \draw [->] (Q) -| (policyQ);
    \draw [<-] (system.west) -- ++(-0.6cm,0) coordinate(p1){};
    \draw [-o] (p1) -- node [pos=0.3] [name=A] [above] {$u_{k}$} ++(-1.1cm,0) coordinate(p2){};
    \draw [-] (p1) |- ++(0,-3.6cm) coordinate(p3);
    \draw [->] (p3) |-  ++(-0.16cm,0) coordinate(p4);
    % \draw [-] (p1) -- ++(0,-0.5cm) coordinate(p2){};
    % \draw [->] (A) |- (RF);
    % \draw [->] (S1) |- (LU);
    % \draw [->] (A) |- (LU);
    % \draw [->] (LU) -- node [pos=0.5] [name=temp] [right] {} (Q);
    % \draw [->] (temp) -| (policyQ);
    % \draw [->] (S1) |- ([xshift=-0.3cm,yshift=-0.27cm]LU.south west) -| (CL);
    % \draw [->] (CL) -- node [pos=0.5] [name=v] [right] {{$v_{k}$}} (policyT);
    \draw [-] (RL) -- node [pos=0.5] [name=A1] [above] {$\pi^{\R{rl}}$} ++ (-2.5cm,0) coordinate(pq1){};
    \draw [-] (pq1) -- ++(0,3.5cm) coordinate(pq2){};
    \draw [-o] (pq2) -- ++(2.2cm,0) coordinate(pq3){};
    \draw [->] (RL.north) -- node [pos=0.5] [name=A2] {$\zeta_k$} ++ (0,2.6cm) coordinate(pq4){};
    
    \draw [-] (CT) -- node [pos=0.3] [name=A3] [above] {$\pi^{\R{c}}$} ++(-3.5cm,0) coordinate(pt1){};
    \draw [-] (pt1) -- ++(0,6cm) coordinate(pt2){};
    \draw [-o] (pt2) -- ++(3.2cm,0) coordinate(pt3){};

    \draw [-] (p2) -- (pq3);
    \draw[<-] ($(pt3)+(0.5cm,0.1cm)$) to [bend right]($(pq3)+(0.5cm,-0.1cm)$);
    % \draw[->]  (pq1)  to [out=-150,in=-30] (pt1);
     
\end{tikzpicture}
\caption{Schematic of the Control-Tutored Reinforcement Learning (CTRL) algorithm.}
%At each time instant $k$, the control action $u_k$ is selected by choosing either the control action suggested by the control-tutor policy $\pi^C$ or the one suggested by the RL policy $\pi^R$.} %The choice is made in accordance to a boolean variable, $\zeta$, that will be formally defined in Section \ref{sec:CTQL}.} 
\label{fig:CTQL}
\vspace{-0.5cm}
\end{figure}
